Estimates of Light Quark Masses from Lattice QCD and QCD Sum rules

This talk reviews the progress made in the determination of the light quark masses using lattice QCD and QCD sum rules. Based on preliminary calculations with three flavors of dynamical quarks, the lattice estimate is $m_s = 75(15)$ MeV, a tantalizingly low value. On the other hand the leading estimates from scale and pseudo-scalar sum rules are $99(16)$ and $100(12)$ MeV respectively. The $\tau$-decay sum rule estimates depend very sensitively on the value of $|V_{us}|$. The central values from different analyses lie in the range 115-120 MeV if unitarity of CKM matrix is imposed, and in the range 100-105 MeV if the Particle Data Group values for $|V_{us}|$ are used. I also give my reasons for why the lattice result is not yet in conflict with rigorous lower bounds from sum rule analyses.

==> Makefile <==
LATEX  = latex
BIBTEX = bibtex
DVIPS  = dvips
SHELL  = /bin/sh

# %auto-ignore
MAINFILE=  paper.tex

TEXFILES =  ckm.bst ckm.cls
AXISFILES= CPPACS_mq.ax
FIGFILES =  
PSFILES  = contour.eps logo.eps
#########################################################################
# special rules if any

#########################################################################
#									#
#                 NO USER SERVICEABLE PARTS BELOW !!!                   #
# 									#
#########################################################################


# List of all the sources
SOURCES= Makefile ${MAINFILE} ${TEXFILES} ${AXISFILES} ${FIGFILES} ${PSFILES}

# List of all postscript figures to be included.
PSINCLUSIONS= ${AXISFILES:.ax=.ps} ${FIGFILES:.fig=.ps} ${PSFILES}

# what is to be made by default
all: ${MAINFILE:.tex=.ps}

# re-dvips if any of these change
${MAINFILE:.tex=.ps}: ${MAINFILE:.tex=.dvi} ${PSINCLUSIONS}

# re-latex if any of these change
${MAINFILE:.tex=.dvi}: ${MAIN} ${MAINFILE:.tex=.bbl} ${TEXFILES} ${PSINCLUSIONS}

${MAINFILE:.tex=.bbl}: ${MAIN} ${MAINFILE:.tex=.bib} ${TEXFILES} ${PSINCLUSIONS}
# Never try to `make' any of the sources
${SOURCES}:;

# The rest of them do not have any `extra' dependencies, i.e. a.x depends 
# obviously depends on a.y if a.x is to be created from a.y.

.PHONY: clean realclean
# clean removes ~ aux log and tmp files
clean:
	rm -f *~ *.aux *.log *.tmp
# real clean removes everything but sources and final products
realclean: clean
	rm -f ${AXISFILES:.ax=.ps} ${FIGFILES:.fig=.ps}

########################################################################
# General rules of how to build something from something else.
.SUFFIXES: .ps .dvi .tex .ax .xy .fig

# If .fig exists that is how to create ps.
%.ps: %.fig
	fig2dev -L ps $< > $@

# If .ax or .xy exist, that is the source of the .ps file
%.ps: %.ax
	xyplot $< | epsplot > $@.tmp
	sed -e "s/%%BoundingBox: (atend)/`psbbox $@.tmp | head -1`/p" \
            -e '/%%BoundingBox/d' $@.tmp > $@ 
	rm -f $@.tmp
%.ps: %.xy
	xyplot $< | epsplot > $@.tmp
	sed -e "s/%%BoundingBox: (atend)/`psbbox $@.tmp | head -1`/p" \
            -e '/%%BoundingBox/d' $@.tmp > $@ 
	rm -f $@.tmp

# else look for a dvi file.
%.ps: %.dvi
	$(DVIPS)  $< -o
%.dvi: %.tex
	$(LATEX) $< && $(BIBTEX) $* && $(LATEX) $< && $(LATEX) $<
	-while [ `grep '^Rerun ' $*.log` ]; do $(LATEX) $< ; done

# Save paper
%.ps2: %.ps
	pstops -w21cm -h29.7cm '2:0L@.65(1w,0)+1L@.65(1w,.45h)' $< | sed -e '1a\
	%%Orientation: Landscape' > $@

##################################################################

submission: ${SOURCES} ${PSINCLUSIONS} ${MAINFILE:.tex=.bbl} ${MAINFILE:.tex=.bib}
	rm -f submission.uu
	(echo "."; \
	 echo "${SOURCES} ${PSINCLUSIONS} ${MAINFILE:.tex=.bbl} ${MAINFILE:.tex=.bib}" ; \
	 echo "submission") | uufiles -gz -9


